Modeling Path Importance for Effective Alzheimer's Disease Drug Repurposing

Recently, drug repurposing has emerged as an effective and resource-efficient paradigm for AD drug discovery. Among various methods for drug repurposing, network-based methods have shown promising results as they are capable of leveraging complex networks that integrate multiple interaction types, such as protein-protein interactions, to more effectively identify candidate drugs. However, existing approaches typically assume paths of the same length in the network have equal importance in identifying the therapeutic effect of drugs. Other domains have found that same length paths do not necessarily have the same importance. Thus, relying on this assumption may be deleterious to drug repurposing attempts. In this work, we propose MPI (Modeling Path Importance), a novel network-based method for AD drug repurposing. MPI is unique in that it prioritizes important paths via learned node embeddings, which can effectively capture a network's rich structural information. Thus, leveraging learned embeddings allows MPI to effectively differentiate the importance among paths. We evaluate MPI against a commonly used baseline method that identifies anti-AD drug candidates primarily based on the shortest paths between drugs and AD in the network. We observe that among the top-50 ranked drugs, MPI prioritizes 20.0% more drugs with anti-AD evidence compared to the baseline. Finally, Cox proportional-hazard models produced from insurance claims data aid us in identifying the use of etodolac, nicotine, and BBB-crossing ACE-INHs as having a reduced risk of AD, suggesting such drugs may be viable candidates for repurposing and should be explored further in future studies.

==> tables/baseline.tex <==
\begin{ThreePartTable}
\renewcommand\TPTminimum{\textwidth}
%% Arrange for "longtable" to take up full width of text block
\setlength\LTleft{0pt}
\setlength\LTright{0pt}
\setlength\tabcolsep{3pt}

\centering
\footnotesize

\begin{TableNotes}[normal,flushleft]
%\begin{scriptsize}
    \item {\footnotesize{These columns have the same meaning as those in Table~\ref{tbl:drugs_method}}.}
    \par
%\end{scriptsize}
\end{TableNotes}

\begin{longtable}{l l l c l}
  \caption{Top-50 Drugs from \baseline}
  \label{tbl:drugs_baseline}\\
  \toprule
  Drug & MOA & Indication & Anti-\AD & Evidence\\
  \midrule
  %
  \multirow{2}{*}{tetracycline} & bacterial 30S
  & respiratory tract & \multirow{2}{*}{Y}
  & \multirow{2}{*}{\textit{in vitro}~\cite{forloni2001anti}}\\
  & ribosomal subunit inhibitor & infections &&\\
  %
  selegiline & monoamine oxidase inhibitor & Parkinson's Disease & N & -\\
  %
  \multirow{2}{*}{ceftriaxone} & bacterial cell wall & \multirow{2}{*}{gonorrhea} & \multirow{2}{*}{Y} & \multirow{2}{*}{\textit{in vivo}~\cite{tikhonova2021neuroprotective}}\\
  & synthesis inhibitor &&&\\
  %
  ibuprofen & \coxs & headache & N & -\\
  %
  levobunolol & adrenergic receptor antagonist & glaucoma & N & -\\
  %
  ketoprofen & \coxs & rheumatoid arthritis & N & -\\
  %
  \multirow{2}{*}{carbidopa} & aromatic L-amino acid & \multirow{2}{*}{Parkinson's Disease} & \multirow{2}{*}{N} & \multirow{2}{*}{-}\\
  & decarboxylase inhibitor &&&\\
  %
  sulindac & \coxs & osteoarthritis & Y & \textit{in vivo}~\cite{modi2014sulindac}\\
  %
  biotin & vitamin B & supplement & Y & \textit{in vivo}~\cite{lohr2020biotin}\\
  %
  lansoprazole & ATPase inhibitor & heartburn & N & -\\
  %
   %THIS IS THE CUTOFF -- REMOVE EVERYTHING BELOW%
  %
  itraconazole & cytochrome P450 inhibitor & onychomycosis & N & -\\
  %
  ketorolac & \coxs & pain relief & N & -\\
  %
  quinidine & sodium channel blocker & malaria & N & -\\
  %
  terbinafine & fungal squalene epoxidase inhibitor & tinea pedis & N & -\\
  %
  labetalol & adrenergic receptor antagonist & hypertension & N & -\\
  %
  vilazodone & serotonin reuptake inhibitor & depression & N & -\\
  %
  \multirow{2}{*}{ivermectin} & \multirow{2}{*}{benzodiazepine receptor agonist} & gastrointestinal & \multirow{2}{*}{N} & \multirow{2}{*}{-}\\
  && roundworms &&\\
  %
  \multirow{2}{*}{oxiconazole} & bacterial cell wall & \multirow{2}{*}{tinea pedis} & \multirow{2}{*}{N} & \multirow{2}{*}{-}\\
  & synthesis inhibitor &&&\\
  %
  dabigatran & thrombin inhibitor & stroke & Y & \textit{in vivo}~\cite{cortes2019long}\\
  %
  \multirow{2}{*}{linezolid} & bacterial 50S & \multirow{2}{*}{pneumonia} & \multirow{2}{*}{N} & \multirow{2}{*}{-}\\
  & ribosomal subunit inhibitor &&&\\
  %
  indomethacin & \coxs & rheumatoid arthritis & Y & clinical~\cite{rogers1993clinical}\\
  %
  donepezil & \aches & Alzheimer's disease & Y & approved\\
  %
  levodopa & dopamine precursor & Parkinson's Disease & N & -\\
  %
  ketoconazole & sterol demethylase inhibitor & seborrheic dermatitis & N & -\\
  %
  loratadine & histamine receptor antagonist & allergic rhinitis & N & -\\
  %
  lovastatin & HMGCR inhibitor & coronary heart disease & Y & other~\cite{ransmayr2003cholesterol}\\
  %
  triamterene & sodium channel blocker & hypokalemia & Y & clinical~\cite{triamterene}\\
  %
  captopril & \aces & hypertension & Y & \textit{in vivo}~\cite{abbassi2016captopril}\\
  %
  naproxen & \coxs & pain relief & N & -\\
  %
  methyldopa & adrenergic receptor agonist & hypertension & N & -\\
  %
  \multirow{2}{*}{fluvoxamine} & selective serotonin & obsessive compulsive & \multirow{2}{*}{Y} & \multirow{2}{*}{\textit{in vivo}~\cite{kim2018effect}}\\
  & reuptake inhibitor & disorder &&\\
  %
  zonisamide & sodium channel blocker & seizures & N & -\\
  %
  diflunisal & prostanoid receptor antagonist & rheumatoid arthritis & Y & \textit{in vivo}~\cite{rejc2020oral}\\
  %
  \multirow{2}{*}{sertraline} & selective serotonin &
  \multirow{2}{*}{depression} & \multirow{2}{*}{N} & \multirow{2}{*}{-}\\
  & reuptake inhibitor &&&\\
  %
  rasagiline & monoamine oxidase inhibitor & Parkinson's Disease & Y & clinical~\cite{rasagiline}\\
  %
  verapamil & calcium channel blocker & hypertension & Y & \textit{in vivo}~\cite{ahmed2022repurposing}\\
  %
  metoclopramide & dopamine receptor antagonist & gastroparesis & N & -\\
  %
  diclofenac & \coxs & rheumatoid arthritis & Y & other~\cite{stuve2020diclofenac}\\
  %
  bupropion & dopamine reuptake inhibitor & depression & N & -\\
  %
  amiloride & sodium channel blocker & hypertension & Y & clinical~\cite{triamterene}\\
  %
  vortioxetine & serotonin receptor agonist & depression & N & -\\
  %
  trazodone & adrenergic receptor antagonist & depression & N & -\\
  %
  losartan & angiotensin receptor antagonist & hypertension & N & -\\
  %
  trihexyphenidyl & acetylcholine receptor antagonist & parkinsonism & N & -\\
  %
  \multirow{2}{*}{fluoxetine} & selective serotonin & \multirow{2}{*}{depression} & \multirow{2}{*}{Y} &
  \multirow{2}{*}{\textit{in vivo}~\cite{abu2022fluoxetine}}\\
  & reuptake inhibitor &&&\\
  %
  azelastine & histamine receptor antagonist & conjunctivitis & N & -\\
  %
  nicotine & \acrs
  & smoking cessation & Y & clinical~\cite{newhouse2012nicotine}\\
  %
  dexamethasone & glucocorticoid receptor agonist & hypercalcemia & Y & \textit{in vivo}~\cite{hui2020combination}\\
  %
  \multirow{2}{*}{doxazosin}
  & \multirow{2}{*}{adrenergic receptor antagonist}
  & benign prostatic & \multirow{2}{*}{Y}
  & \multirow{2}{*}{\textit{in vitro}~\cite{coelho2019dual}}\\
  && hyperplasia &&\\
  %
  tramadol & centrally-acting opioid agonist & pain management & N & -\\
  \bottomrule
  \insertTableNotes
\end{longtable}
\end{ThreePartTable}

==> tables/method.tex <==
\begin{ThreePartTable}
\renewcommand\TPTminimum{\textwidth}
%% Arrange for "longtable" to take up full width of text block
\setlength\LTleft{0pt}
\setlength\LTright{0pt}
\setlength\tabcolsep{3pt}

\centering
\footnotesize

\begin{TableNotes}[normal, flushleft]
\item{\footnotesize{In this table, the column ``Drug" shows the identified top-50 ranked drugs; the column ``MOA" shows the mechanism of action of each drug; the column ``Indication" presents the indication of each drug;
the column ``Anti-\AD" indicates if the drug has evidenced anti-\AD effects;
and the column ``Evidence" presents the type of the evidence.
%
In this table, \aces represents the angiotensin converting enzyme inhibitor;
\coxs represents the cyclooxygenase inhibitor;
\aches represents the acetylcholinesterase inhibitor;
and \acrs represents the acetylcholine receptor agonist.}}
\par
\end{TableNotes}

\begin{longtable}{l l l c l}
  \caption{Top-50 Drugs from \method}
  \label{tbl:drugs_method}\\
      \toprule
      Drug & MOA & Indication & Anti-\AD & Evidence\\
      \midrule
      %
      varenicline & \acrs & smoking cessation & N & -\\
      %
      fosinopril &
      \aces & hypertension & Y & \textit{in vivo}~\cite{deb2015comparative}\\
      %
      nicotine & \acrs
      & smoking cessation & Y & clinical~\cite{newhouse2012nicotine}\\
      %
      nizatidine & histamine receptor antagonist & duodenal ulcer disease & N & -\\
      %
      piroxicam & \coxs & osteoarthritis & Y & other~\cite{zhang2018nsaid,imbimbo2010nsaids}\\
      %
      meloxicam & \coxs & osteoarthritis & Y & \textit{in vivo}~\cite{ianiski2016meloxicam,guan2023meloxicam,ianiski2012protective}\\
      %
      galantamine & \aches & Alzheimer's disease & Y & approved\\
      %
      bromfenac & \coxs & inflammation & N & -\\
      %
      etodolac & \coxs & osteoarthritis & Y & \textit{in vivo}~\cite{elfakhri2019multi}\\
      %
      pyridostigmine & \aches & myasthenia gravis & N & -\\
      %
      %THIS IS THE CUTOFF -- REMOVE EVERYTHING BELOW%
      %
      bupropion & dopamine reuptake inhibitor & depression & N & -\\
      %
      pentoxifylline & phosphodiesterase inhibitor & claudication & N & -\\
      %
      flurbiprofen & \coxs & rheumatoid arthritis & Y & clinical~\cite{geerts2007drug}\\
      %
      zonisamide & sodium channel blocker & seizures & N & -\\
      %
      apixaban & coagulation factor inhibitor & stroke & Y & other~\cite{zhang2018nsaid,imbimbo2010nsaids}\\
      %
      rivastigmine & \aches & Alzheimer's disease & Y & approved\\
      %
      ramipril & \aces & hypertension & Y & clinical~\cite{wharton2012effects}\\
      %
      \multirow{2}{*}{linezolid} & bacterial 50S & \multirow{2}{*}{pneumonia} & \multirow{2}{*}{N} & \multirow{2}{*}{-}\\
      & ribosomal subunit inhibitor &&&\\
      %
      trandolapril & \aces & hypertension & Y & \textit{in vivo}~\cite{wang2013unintended}\\
      %
      moexipril & \aces & hypertension & N & -\\
      %
      quinapril & \aces & hypertension & N & -\\
      %
      enalapril & \aces & hypertension & N & -\\
      %
      benazepril & \aces & hypertension & N & -\\
      %
      lisinopril & \aces & hypertension & Y & \textit{in vivo}~\cite{thomas2021angiotensin}\\
      %
      hydralazine & vasodilator & hypertension & Y & \textit{in vitro}~\cite{maheshwari2010hydralazine}\\
      %
      rasagiline & monoamine oxidase inhibitor & Parkinson's Disease & Y & clinical~\cite{rasagiline}\\
      %
      ganciclovir & DNA polymerase inhibitor & cytomegalovirus & Y & \textit{in vivo}~\cite{katsouri2020ablation}\\
      %
      naproxen & \coxs & pain relief & N & -\\
      %
      \multirow{2}{*}{fluvoxamine} & selective serotonin & obsessive compulsive & \multirow{2}{*}{Y} & \multirow{2}{*}{\textit{in vivo}~\cite{kim2018effect}}\\
      & reuptake inhibitor & disorder &&\\
      %
      dapsone & bacterial antifolate & dermatitis herpetiformis & Y & other~\cite{lee2022dapsone}\\
      %
      oxaprozin & \coxs & osteoarthritis & Y & other~\cite{zhang2018nsaid,imbimbo2010nsaids}\\
      %
      ranitidine & histamine receptor antagonist & heartburn & N & -\\
      %
      donepezil & \aches & Alzheimer's disease & Y & approved\\
      %
      memantine & glutamate receptor antagonist & Alzheimer's disease & Y & approved\\
      %
      \multirow{2}{*}{empagliflozin} &
      sodium/glucose cotransporter & diabetes &
      \multirow{2}{*}{Y} & \multirow{2}{*}{\textit{in vivo}~\cite{hierro2020empagliflozin}}\\
      & inhibitor & mellitus && \\
      %
      \multirow{2}{*}{canagliflozin} &
      sodium/glucose cotransporter & diabetes &
      \multirow{2}{*}{N} & \multirow{2}{*}{-}\\
      & inhibitor & mellitus && \\
      %
      alogliptin & dipeptidyl peptidase inhibitor
      & diabetes mellitus & Y & \textit{in vivo}~\cite{rahman2020alogliptin,el2021alogliptin}\\
      %
      \multirow{2}{*}{oxiconazole} & bacterial cell wall
      & \multirow{2}{*}{tinea pedis} & \multirow{2}{*}{N} & \multirow{2}{*}{-}\\
      & synthesis inhibitor &&&\\
      %
      rivaroxaban & coagulation factor inhibitor & stroke & Y & \textit{in vivo}~\cite{bian2022protective}\\
      %
      \multirow{2}{*}{fluoxetine} & selective serotonin & \multirow{2}{*}{depression} & \multirow{2}{*}{Y} &
      \multirow{2}{*}{\textit{in vivo}~\cite{abu2022fluoxetine}}\\
      & reuptake inhibitor &&&\\
      %
      azelastine & histamine receptor antagonist & conjunctivitis & N & -\\
      %
      \multirow{2}{*}{sertraline} & selective serotonin &
      \multirow{2}{*}{depression} & \multirow{2}{*}{N} & \multirow{2}{*}{-}\\
      & reuptake inhibitor &&&\\
      %
      ibuprofen & \coxs & headache & N & -\\
      %
      labetalol & adrenergic receptor antagonist & hypertension & N & -\\
      %
      \multirow{2}{*}{duloxetine} & norepinephrine reuptake & \multirow{2}{*}{depression} & \multirow{2}{*}{N} & \multirow{2}{*}{-}\\
      & inhibitor &&&\\
      %
      \multirow{2}{*}{quinine} & hemozoin biocrystallization & \multirow{2}{*}{malaria} & \multirow{2}{*}{N} & \multirow{2}{*}{-}\\
      & inhibitor &&&\\
      %
      trihexyphenidyl & acetylcholine receptor antagonist & parkinsonism & N & -\\
      %
      ketoprofen & \coxs & rheumatoid arthritis & N & -\\
      %
      selegiline & monoamine oxidase inhibitor & Parkinson's Disease & N & -\\
      %
      nortriptyline & tricyclic antidepressant & depression & N & -\\
      \bottomrule
      \insertTableNotes
\end{longtable}
\end{ThreePartTable}
